SN4KE: Practical Mutation Testing at Binary Level

Mutation analysis is an effective technique to evaluate a test suite adequacy in terms of revealing unforeseen bugs in software. Traditional source- or IR-level mutation analysis is not applicable to the software only available in binary format. This paper proposes a practical binary mutation analysis via binary rewriting, along with a rich set of mutation operators to represent more realistic bugs. We implemented our approach using two state-of-the-art binary rewriting tools and evaluated its effectiveness and scalability by applying them to SPEC CPU benchmarks. Our analysis revealed that the richer mutation operators contribute to generating more diverse mutants, which, compared to previous works leads to a higher mutation score for the test harness. We also conclude that the reassembleable disassembly rewriting yields better scalability in comparison to lifting to an intermediate representation and performing a full translation.

==> tables/capstone-grp.tex <==
% \resizebox{\columnwidth}{!}{
\begin{tabular}{ll}
\hline \toprule
Mutation Class              & Description        \\
\midrule
\midrule
\multirow{2}{*}{Arithmetic} & Replace arithmetic assignment operators from the set of \{+=, -+, *=, /=\}           \\
                            & Replace with an operator from the set of \{+, -, *, /, \%\}                          \\
\midrule
\multirow{3}{*}{Logical}           & Substitute with another bit-wise logical operator from \{\textasciicircum{}, \mid, \&\} \\
                            & replace with a logical assignment from \{\textasciicircum{}=, \mid=, \&=\}              \\
                            & Substitute the connector with another logical operator from \{\&\&, \parallel\}   \\
\midrule
\multirow{2}{*}{Conditional}           & Substitute any conditional jump with an unconditional branch to force taking the branch \\
                            & taking the fall-through (instruction following the branch) edge of branch by NOPing the condition   \\
\midrule
Constants           &   Replace any immediate value \textit{c} with one another constant from set \{-1, 0, 1, -c, c+1, c-1\} \\
\midrule
Skip                &   Replace instructions from set Arithmetic, Logical, and Conditional with a NOP operator to skip the execution of that operator
\midrule
\bottomrule
\end{tabular}
% }



==> tables/tbl_spec_results.tex <==
\begin{tabular}{lll}
\hline \toprule
\textbf{Benchmark} & \textbf{Description} & \textbf{Trivial Input} \\
\midrule
\midrule
gcc	&	C Compiler &An empty .i file \\
\midrule
gobmk	&  Go game playing & An empty game (.sgf file) \\
\midrule
perlbench	& PERL Programming Language & An empty .pl file \\
\midrule
h264ref	& Video Compression & No input file \\
\midrule
hmmer		& Search Gene Sequence& -h \\	
\midrule
sphinx	& Speech recognition & -h \\
\midrule
sjeng		& Artificial Intelligence: chess &  Analyze a potision to  depth 0 \\
\midrule
milc		& Physics: Quantum Chromodynamics & A grid of size 0 \\
\midrule
bzip2		& Compression & An empty file, with compression level 0 \\
\midrule
libquantum	&Physics: Quantum Computing & -h \\
\midrule
lbm	& Fluid Dynamics & Time step 0 \\
\midrule
mcf	& Vehicle scheduling & 0 trips \\
\bottomrule

\end{tabular}
